Quantum Control of Interacting Bosons in Periodic Optical Lattice

We study the avoided crossings in the dynamics of quantum controlled excitations for an interacting two-boson system in an optical lattice. Specifically, we perform numerical simulations of quantum control in this system where driving pulses connect the undriven stationary states in a manner characteristic of Stimulated Raman Adiabatic Passage (STIRAP). We demonstrate that the dynamics of such a transition is affected by chaos induced avoided crossings, resulting in a loss in coherence of the final outcome in the adiabatic limit.

==> zzclean <==
#!/bin/sh
#
#	mydiss/zzclean
#
#
rm -f	*~ \
	*.blg \
	*.dvi \
	*.idx \
	*.ilg \
	*.ind \
	*.log \
	*.lot \
	*.ps  \
	*.pdf \
	*.backup \
	*.toc   2>/dev/null


